KG-ECO: Knowledge Graph Enhanced Entity Correction for Query Rewriting

Query Rewriting (QR) plays a critical role in large-scale dialogue systems for reducing frictions. When there is an entity error, it imposes extra challenges for a dialogue system to produce satisfactory responses. In this work, we propose KG-ECO: Knowledge Graph enhanced Entity COrrection for query rewriting, an entity correction system with corrupt entity span detection and entity retrieval/re-ranking functionalities. To boost the model performance, we incorporate Knowledge Graph (KG) to provide entity structural information (neighboring entities encoded by graph neural networks) and textual information (KG entity descriptions encoded by RoBERTa). Experimental results show that our approach yields a clear performance gain over two baselines: utterance level QR and entity correction without utilizing KG information. The proposed system is particularly effective for few-shot learning cases where target entities are rarely seen in training or there is a KG relation between the target entity and other contextual entities in the query.

==> refs_full.tex <==
@InProceedings{C2,
  author = 	 "Jones, C.D. and Smith, A.B. and Roberts, E.F.",
  title =        "Article Title",
  booktitle =        "Proceedings Title",
  organization = "IEEE",
  year = 	 "2003",
  volume = 	 "II",
  pages = 	 "803-806"
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Use this file for citations not found in the ACL Anthology (contained in "anthology.bib").

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Query Rewriting

@article{He2016,
    author = {He, Yunlong and Tang, Jiliang and Ouyang, Hua and Kang, Changsung and Yin, Dawei and Chang, Yi},
    doi = {10.1145/2983323.2983835},
    isbn = {9781450340731},
    journal = {CIKM '16: Proceedings of the 25th ACM International on Conference on Information and Knowledge Management},
    title = {Learning to Rewrite Queries},
    url = {http://dx.doi.org/10.1145/2983323.2983835},
    year = {2016}
}

@article{Ponnusamy2020, 
    title={Feedback-Based Self-Learning in Large-Scale Conversational AI Agents}, 
    volume={34}, 
    url={https://ojs.aaai.org/index.php/AAAI/article/view/7022}, 
    DOI={10.1609/aaai.v34i08.7022}, 
    number={08}, 
    journal={Proceedings of the AAAI Conference on Artificial Intelligence}, 
    author={Ponnusamy, Pragaash and Roshan Ghias, Alireza and Guo, Chenlei and Sarikaya, Ruhi}, 
    year={2020}, 
    month={Apr.}, 
    pages={13180-13187}
}


@article{Chen2020,
   author = {Zheng Chen and Xing Fan and Yuan Ling and Lambert Mathias and Chenlei Guo},
   journal = {ICASSP, IEEE International Conference on Acoustics, Speech and Signal Processing - Proceedings},
   title = {Pre-Training for Query Rewriting in A Spoken Language Understanding System},
   url = {http://dx.doi.org/10.1109/ICASSP40776.2020.9053531},
   year = {2020},
}


@article{Fan2021,
   author = {Xing Fan and Eunah Cho and Xiaojiang Huang and Chenlei Guo},
   journal = {In 2nd International Workshop on Data-Efficient Machine Learning (DeMaL)},
   keywords = {Query rewrite,Search,Self-learning,Spoken dialogue system},
   title = {Search based Self-Learning Query Rewrite System in Conversational AI},
   year = {2021},
}

@article{Yuan2021,
   author = {Siyang Yuan and Saurabh Gupta and Xing Fan and Derek Liu and Yang Liu and Chenlei Guo},
   journal = {ICASSP, IEEE International Conference on Acoustics, Speech and Signal Processing - Proceedings},
   title = {GRAPH ENHANCED QUERY REWRITING FOR SPOKEN LANGUAGE UNDERSTANDING SYSTEM},
   url = {http://dx.doi.org/10.1109/ICASSP39728.2021.9413840},
   year = {2021},
}

@inproceedings{Cho2021,
    title = "Personalized Search-based Query Rewrite System for Conversational {AI}",
    author = "Cho, Eunah  and
      Jiang, Ziyan  and
      Hao, Jie  and
      Chen, Zheng  and
      Gupta, Saurabh  and
      Fan, Xing  and
      Guo, Chenlei",
    booktitle = "Proceedings of the 3rd Workshop on Natural Language Processing for Conversational AI",
    month = nov,
    year = "2021",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.nlp4convai-1.17",
    doi = "10.18653/v1/2021.nlp4convai-1.17",
    pages = "179--188",
}


@inproceedings{WangZ2021,
    title = "Contextual Rephrase Detection for Reducing Friction in Dialogue Systems",
    author = "Wang, Zhuoyi  and
      Gupta, Saurabh  and
      Hao, Jie  and
      Fan, Xing  and
      Li, Dingcheng  and
      Li, Alexander Hanbo  and
      Guo, Chenlei",
    booktitle = "Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing (EMNLP)",
    month = nov,
    year = "2021",
    address = "Online and Punta Cana, Dominican Republic",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.emnlp-main.143",
    doi = "10.18653/v1/2021.emnlp-main.143",
    pages = "1899--1905",
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% KG/Entity correction/linking...


@article{Fu2020,
    archivePrefix = {arXiv},
    arxivId = {2007.13069},
    author = {Fu, Bin and Qiu, Yunqi and Tang, Chengguang and Li, Yang and Yu, Haiyang and Sun, Jian},
    eprint = {2007.13069},
    journal = {arXiv},
    month = {jul},
    title = {{A Survey on Complex Question Answering over Knowledge Base: Recent Advances and Challenges}},
    url = {http://arxiv.org/abs/2007.13069},
    year = {2020}
}


@article{Guo2020,
    archivePrefix = {arXiv},
    arxivId = {2003.00911},
    author = {Guo, Qingyu and Zhuang, Fuzhen and Qin, Chuan and Zhu, Hengshu and Xie, Xing and Xiong, Hui and He, Qing},
    eprint = {2003.00911},
    journal = {arXiv},
    month = {feb},
    title = {{A Survey on Knowledge Graph-Based Recommender Systems}},
    url = {http://arxiv.org/abs/2003.00911},
    year = {2020}
}


@inproceedings{WuL2020,
    title = "Scalable Zero-shot Entity Linking with Dense Entity Retrieval",
    author = "Wu, Ledell  and
      Petroni, Fabio  and
      Josifoski, Martin  and
      Riedel, Sebastian  and
      Zettlemoyer, Luke",
    booktitle = "Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.emnlp-main.519",
    doi = "10.18653/v1/2020.emnlp-main.519",
    pages = "6397--6407",
}


@article{WuJ2020,
   author = {Junshuang Wu and Richong Zhang and Yongyi Mao and Hongyu Guo and Masoumeh Soflaei and Jinpeng Huai},
   journal = {The Web Conference - Proceedings of the World Wide Web Conference, WWW},
   title = {Dynamic Graph Convolutional Networks for Entity Linking},
   url = {https://doi.org/10.1145/3366423.3380192},
   year = {2020},
}


@inproceedings{Raghuvanshi2019,
    title = "Entity resolution for noisy {ASR} transcripts",
    author = "Raghuvanshi, Arushi  and
      Ramakrishnan, Vijay  and
      Embar, Varsha  and
      Carroll, Lucien  and
      Raghunathan, Karthik",
    booktitle = "Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP): System Demonstrations",
    month = nov,
    year = "2019",
    address = "Hong Kong, China",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/D19-3011",
    doi = "10.18653/v1/D19-3011",
    pages = "61--66",
}

@article{WangH2020,
   author = {Haoyu Wang and Shuyan Dong and Yue Liu and James Logan and Ashish Kumar Agrawal and Yang Liu},
   journal = {Proceedings of the Annual Conference of the International Speech Communication Association, INTERSPEECH},
   title = {ASR Error Correction with Augmented Transformer for Entity Retrieval},
   year = {2020},
}

@inproceedings{Muralidharan2021,
    title = "Noise Robust Named Entity Understanding for Voice Assistants",
    author = "Muralidharan, Deepak  and
      Moniz, Joel Ruben Antony  and
      Gao, Sida  and
      Yang, Xiao  and
      Kao, Justine  and
      Pulman, Stephen  and
      Kothari, Atish  and
      Shen, Ray  and
      Pan, Yinying  and
      Kaul, Vivek  and
      Seyed Ibrahim, Mubarak  and
      Xiang, Gang  and
      Dun, Nan  and
      Zhou, Yidan  and
      O, Andy  and
      Zhang, Yuan  and
      Chitkara, Pooja  and
      Wang, Xuan  and
      Patel, Alkesh  and
      Tayal, Kushal  and
      Zheng, Roger  and
      Grasch, Peter  and
      Williams, Jason D  and
      Li, Lin",
    booktitle = "Proceedings of the 2021 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies: Industry Papers",
    month = jun,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.naacl-industry.25",
    doi = "10.18653/v1/2021.naacl-industry.25",
    pages = "196--204",
}

@article{WangH2021,
   author = {Haoyu Wang and John Chen and Majid Laali and Kevin Durda and Jeff King and William Campbell and Yang Liu},
   journal = {Proceedings of the Annual Conference of the International Speech Communication Association, INTERSPEECH},
   title = {Leveraging ASR N-best in Deep Entity Retrieval},
   year = {2021},
}

@inproceedings{WangT2021,
    title = "Optimizing {NLU} Reranking Using Entity Resolution Signals in Multi-domain Dialog Systems",
    author = "Wang, Tong  and
      Chen, Jiangning  and
      Malmir, Mohsen  and
      Dong, Shuyan  and
      He, Xin  and
      Wang, Han  and
      Su, Chengwei  and
      Liu, Yue  and
      Liu, Yang",
    booktitle = "Proceedings of the 2021 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies: Industry Papers",
    month = jun,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.naacl-industry.3",
    doi = "10.18653/v1/2021.naacl-industry.3",
    pages = "19--25",
}


% entity retrieval/resolution/understanding with noisy input

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% GNN

@article{Velickivic2018,
   author = {Petar Veli{\v c}kovi{\'c} and Arantxa Casanova and Pietro Li{\`o} and Guillem Cucurull and Adriana Romero and Yoshua Bengio},
   journal = {International Conference on Learning Representations (ICLR)},
   title = {Graph attention networks},
   url ={https://iclr.cc/Conferences/2018/Schedule?showEvent=299},
   year = {2018},
}


@inproceedings{Vashishth2020,
    title={Composition-based Multi-Relational Graph Convolutional Networks},
    author={Shikhar Vashishth and Soumya Sanyal and Vikram Nitin and Partha Talukdar},
    booktitle={International Conference on Learning Representations},
    year={2020},
    url={https://openreview.net/forum?id=BylA_C4tPr}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Transformers

@inproceedings{Devlin2018,
    title = "{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding",
    author = "Devlin, Jacob  and
      Chang, Ming-Wei  and
      Lee, Kenton  and
      Toutanova, Kristina",
    booktitle = "Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)",
    month = jun,
    year = "2019",
    address = "Minneapolis, Minnesota",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/N19-1423",
    doi = "10.18653/v1/N19-1423",
    pages = "4171--4186",
}


@article{Liu2019,
    archivePrefix = {arXiv},
    arxivId = {1907.11692},
    author = {Liu, Yinhan and Ott, Myle and Goyal, Naman and Du, Jingfei and Joshi, Mandar and Chen, Danqi and Levy, Omer and Lewis, Mike and Zettlemoyer, Luke and Stoyanov, Veselin},
    eprint = {1907.11692},
    journal = {arXiv},
    month = {jul},
    title = {{RoBERTa: A Robustly Optimized BERT Pretraining Approach}},
    url = {https://arxiv.org/abs/1907.11692v1},
    year = {2019}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Misc

@article{Johnson2017,
  author={Johnson, Jeff and Douze, Matthijs and Jégou, Hervé},
  journal={IEEE Transactions on Big Data}, 
  title={Billion-Scale Similarity Search with GPUs}, 
  year={2021},
  volume={7},
  number={3},
  pages={535-547},
  doi={10.1109/TBDATA.2019.2921572}
}


@inproceedings{Karpukhin2020,
    title = "Dense Passage Retrieval for Open-Domain Question Answering",
    author = "Karpukhin, Vladimir  and
      Oguz, Barlas  and
      Min, Sewon  and
      Lewis, Patrick  and
      Wu, Ledell  and
      Edunov, Sergey  and
      Chen, Danqi  and
      Yih, Wen-tau",
    booktitle = "Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.emnlp-main.550",
    doi = "10.18653/v1/2020.emnlp-main.550",
    pages = "6769--6781",
}


@inproceedings{Gillick2019,
    title = "Learning Dense Representations for Entity Retrieval",
    author = "Gillick, Daniel  and
      Kulkarni, Sayali  and
      Lansing, Larry  and
      Presta, Alessandro  and
      Baldridge, Jason  and
      Ie, Eugene  and
      Garcia-Olano, Diego",
    booktitle = "Proceedings of the 23rd Conference on Computational Natural Language Learning (CoNLL)",
    month = nov,
    year = "2019",
    address = "Hong Kong, China",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/K19-1049",
    doi = "10.18653/v1/K19-1049",
    pages = "528--537",
}

